A fast and sound tagging method for discontinuous named-entity recognition

We introduce a novel tagging scheme for discontinuous named entity recognition based on an explicit description of the inner structure of discontinuous mentions. We rely on a weighted finite state automaton for both marginal and maximum a posteriori inference. As such, our method is sound in the sense that (1) well-formedness of predicted tag sequences is ensured via the automaton structure and (2) there is an unambiguous mapping between well-formed sequences of tags and (discontinuous) mentions. We evaluate our approach on three English datasets in the biomedical domain, and report comparable results to state-of-the-art while having a way simpler and faster model.

==> 9.algorithms.tex <==
\section{Python implementation}
\label{app:implem}

\begin{algorithm*}[t]
    \input{algorithms/viterbi}
    \caption{Viterbi}
    \label{alg:viterbi}
\end{algorithm*}
\begin{algorithm*}[t]
    \input{algorithms/forward}
    \caption{Forward}
    \label{alg:forward}
\end{algorithm*}


==> algorithms/forward.tex <==
\begin{lstlisting}[language=Python]
# tr_weights is a numpy matrix of shape (number of words x 22)
def log_partition(tr_weights):
    num_words = tr_weights.shape[0]

    # Variable for the wavefront of the Forward chart
    inf = torch.tensor(float("-inf"), device=tag_weights.device)
    chart = tag_weights[0].where(INITS, inf)
    
    for i in range(1, num_words):
        t = chart.unsqueeze(0) + tag_weights[i].unsqueeze(1)
        chart = logsumexp(t.where(self.valid_transitions, inf),axis=1)
    
    return logsumexp(chart.where(self.goals, inf), axis=0)
\end{lstlisting}





==> algorithms/viterbi.tex <==
\begin{lstlisting}[language=Python]
# tr_weights is a numpy matrix of shape (number of words x 22)
def argmax(tr_weights):
    num_words = transition_weights.shape[0]
    
    # Copy and detach so we can use backprop to compute the argmax
    tr_weights = tr_weights.detach().requires_grad_(True)
    
    # Viterbi chart: the computation graph takes care of the chart,
    # but we need a variable to reference the wavefront
    inf = torch.tensor(float("-inf"), device=tag_weights.device)
    chart = tr_weights[0].where(INITS, inf)
    
    for i in range(1, num_words):  # loop over words
        t = chart.unsqueeze(0) + tr_weights[i].unsqueeze(1)
        chart = t.where(TR_MATRIX, inf).max(axis=1).values
    
    # get the score of the best path
    # and call backprop to get the best state sequence
    score = chart.where(FINALS, inf).max(axis=0).values.backward()
    return transition_weights.grad.detach().argmax(axis=1)
\end{lstlisting}

==> app_deduction.tex <==
\section{Deduction rules}

Items are of the form $[i, T, T', p, p', p'']$


Axioms:
\begin{itemize}
    \item $[1, \textsc{O}, -, -, -, -]$
    \item $[1, \textsc{B-Cont}, -, -, -, -]$
    \item $[1, \textsc{B-Disc}, \textsc{B-X}, \top, \bot, \bot]$
    \item $[1, \textsc{B-Disc}, \textsc{B-Y}, \bot, \top, \bot]$
\end{itemize}

\begin{prooftree}
    \AxiomC{$[i-1, \textsc{B-Cont}, -, -, -, -]$}
    \UnaryInfC{$[i, \textsc{I-Cont}, -, -, -, -]$}
\end{prooftree}
\begin{prooftree}
    \AxiomC{$[i-1, \textsc{I-Cont}, -, -, -, -]$}
    \UnaryInfC{$[i, \textsc{I-Cont}, -, -, -, -]$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{$[i-1, \textsc{B-Cont}, -, -, -, -]$}
    \UnaryInfC{$[i, \textsc{O}, -, -, -, -]$}
\end{prooftree}
\begin{prooftree}
    \AxiomC{$[i-1, \textsc{I-Cont}, -, -, -, -]$}
    \UnaryInfC{$[i, \textsc{O}, -, -, -, -]$}
\end{prooftree}
\begin{prooftree}
    \AxiomC{$[i-1, \textsc{O}, -, -, -, -]$}
    \UnaryInfC{$[i, \textsc{O}, -, -, -, -]$}
\end{prooftree}

\begin{prooftree}
    \AxiomC{$[i-1, \textsc{B-Cont}, -, -, -, -]$}
    \UnaryInfC{$[i, \textsc{B-Cont}, -, -, -, -]$}
\end{prooftree}
\begin{prooftree}
    \AxiomC{$[i-1, \textsc{I-Cont}, -, -, -, -]$}
    \UnaryInfC{$[i, \textsc{B-Cont}, -, -, -, -]$}
\end{prooftree}
\begin{prooftree}
    \AxiomC{$[i-1, \textsc{O}, -, -, -, -]$}
    \UnaryInfC{$[i, \textsc{B-Cont}, -, -, -, -]$}
\end{prooftree}

==> figures/bio_filtered.tex <==
 \begin{tikzpicture}[
    shorten >=1pt,
    auto,
    > = Latex,
    % scaling
    scale=0.8,
    every node/.style={
        scale=0.6,
        inner sep=0em
    },
    emission/.style={
        sloped,at end,anchor=south east,inner sep=0.2em
    }
]

\node[state]  (q_1) at (0, 0) {$1$};

\node[state]  (q_2) at (2, 2) {$2$};
\node[state]  (q_3) at (2, 0) {$3$};
\node[state]  (q_4) at (2, -2) {$4$};

\node[state]  (q_5) at (4, 2) {$5$};
\node[state]  (q_6) at (4, 0) {$6$};
\node[state]  (q_7) at (4, -2) {$7$};

\node[state,accepting]  (q_8) at (6, 2) {$8$};
\node[state,accepting]  (q_9) at (6, 0) {$9$};
\node[state,accepting]  (q_10) at (6, -2) {$10$};

\node (start) at (-1, 0) {};
\path[->] (start) edge (q_1);

\path[->] (q_1) edge node[emission] {\textsc{O}~~~~~~} (q_2);
\path[->] (q_1) edge node[emission] {\textsc{B}~~~~} (q_3);
%\path[->] (q_1) edge node[emission] {\textsc{I}~~~~~~} (q_4);

%%%%%%%%%

\path[->] (q_2) edge node[emission] {\textsc{O}~~~~~~} (q_5);
\path[->] (q_2) edge node[emission] {\textsc{B}~~~~} (q_6);
%\path[->] (q_2) edge node[emission] {\textsc{I}~~~~~~} (q_7);

\path[->] (q_3) edge node[emission] {\textsc{O}~~~~~~} (q_5);
\path[->] (q_3) edge node[emission] {\textsc{B}~~~~} (q_6);
\path[->] (q_3) edge node[emission,anchor=north east] {\textsc{I}~~~~~~} (q_7);

\path[->] (q_4) edge node[emission,anchor=north east] {\textsc{O}~~~~~~} (q_5);
\path[->] (q_4) edge node[emission,anchor=north east] {\textsc{B}~~~~} (q_6);
\path[->] (q_4) edge node[emission] {\textsc{I}~~~~~~} (q_7);

%%%%%%%

\path[->] (q_5) edge node[emission] {\textsc{O}~~~~~~} (q_8);
\path[->] (q_5) edge node[emission] {\textsc{B}~~~~} (q_9);
%\path[->] (q_5) edge node[emission] {\textsc{I}~~~~~~} (q_10);

\path[->] (q_6) edge node[emission] {\textsc{O}~~~~~~} (q_8);
\path[->] (q_6) edge node[emission] {\textsc{B}~~~~} (q_9);
\path[->] (q_6) edge node[emission,anchor=north east] {\textsc{I}~~~~~~} (q_10);

\path[->] (q_7) edge node[emission,anchor=north east] {\textsc{O}~~~~~~} (q_8);
\path[->] (q_7) edge node[emission,anchor=north east] {\textsc{B}~~~~} (q_9);
\path[->] (q_7) edge node[emission] {\textsc{I}~~~~~~} (q_10);

\end{tikzpicture}

==> figures/bio_full.tex <==
 \begin{tikzpicture}[
    shorten >=1pt,
    auto,
    > = Latex,
    % scaling
    scale=0.8,
    every node/.style={
        scale=0.6,
        inner sep=0em
    },
    emission/.style={
        sloped,at end,anchor=south east,inner sep=0.2em
    }
]

\node[state]  (q_1) at (0, 0) {$1$};

\node[state]  (q_2) at (2, 2) {$2$};
\node[state]  (q_3) at (2, 0) {$3$};
\node[state]  (q_4) at (2, -2) {$4$};

\node[state]  (q_5) at (4, 2) {$5$};
\node[state]  (q_6) at (4, 0) {$6$};
\node[state]  (q_7) at (4, -2) {$7$};

\node[state,accepting]  (q_8) at (6, 2) {$8$};
\node[state,accepting]  (q_9) at (6, 0) {$9$};
\node[state,accepting]  (q_10) at (6, -2) {$10$};

\node (start) at (-1, 0) {};
\path[->] (start) edge (q_1);

\path[->] (q_1) edge node[emission] {\textsc{O}~~~~~~} (q_2);
\path[->] (q_1) edge node[emission] {\textsc{B}~~~~} (q_3);
\path[->] (q_1) edge node[emission] {\textsc{I}~~~~~~} (q_4);

%%%%%%%%%

\path[->] (q_2) edge node[emission] {\textsc{O}~~~~~~} (q_5);
\path[->] (q_2) edge node[emission] {\textsc{B}~~~~} (q_6);
\path[->] (q_2) edge node[emission] {\textsc{I}~~~~~~} (q_7);

\path[->] (q_3) edge node[emission] {\textsc{O}~~~~~~} (q_5);
\path[->] (q_3) edge node[emission] {\textsc{B}~~~~} (q_6);
\path[->] (q_3) edge node[emission,anchor=north east] {\textsc{I}~~~~~~} (q_7);

\path[->] (q_4) edge node[emission,anchor=north east] {\textsc{O}~~~~~~} (q_5);
\path[->] (q_4) edge node[emission,anchor=north east] {\textsc{B}~~~~} (q_6);
\path[->] (q_4) edge node[emission] {\textsc{I}~~~~~~} (q_7);

%%%%%%%

\path[->] (q_5) edge node[emission] {\textsc{O}~~~~~~} (q_8);
\path[->] (q_5) edge node[emission] {\textsc{B}~~~~} (q_9);
\path[->] (q_5) edge node[emission] {\textsc{I}~~~~~~} (q_10);

\path[->] (q_6) edge node[emission] {\textsc{O}~~~~~~} (q_8);
\path[->] (q_6) edge node[emission] {\textsc{B}~~~~} (q_9);
\path[->] (q_6) edge node[emission,anchor=north east] {\textsc{I}~~~~~~} (q_10);

\path[->] (q_7) edge node[emission,anchor=north east] {\textsc{O}~~~~~~} (q_8);
\path[->] (q_7) edge node[emission,anchor=north east] {\textsc{B}~~~~} (q_9);
\path[->] (q_7) edge node[emission] {\textsc{I}~~~~~~} (q_10);

\end{tikzpicture}

==> figures/bio_grammar.tex <==
 \begin{tikzpicture}[
    shorten >=1pt,
    node distance=2cm,
    auto,
    > = triangle 45,
    % scaling
    scale=0.8,
    every node/.style={scale=0.8}
]

\node[state,accepting]  (q_1) at (0, 0) {$1$};
\node[state]  (q_2) at (0, 2) {$2$};

\node (start) at (-1.5, 0) {};
\path[->] (start) edge (q_1);

\path[->] (q_1) edge[bend left] node {\textsc{B}} (q_2);
\path[->] (q_2) edge[bend left] node {$\epsilon$} (q_1);
\path[->] (q_2) edge[loop above] node {\textsc{I}} (q_2);
\path[->] (q_1) edge[loop below] node {\textsc{O}} (q_1);

\end{tikzpicture}

==> tables/results_all.tex <==

\begin{tabular}{@{}l@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{}}
\toprule
& \multicolumn{3}{c}{\cadec} & \multicolumn{3}{c}{\sha} & \multicolumn{3}{c}{\shb} \\
\cmidrule(l{0pt}r{2pt}){2-4}\cmidrule(l{2pt}r{2pt}){5-7}\cmidrule(l{2pt}r{0pt}){8-10}
\\
& P & R & F1
& P & R & F1
& P & R & F1
\\

\midrule
\multicolumn{10}{l}{\textbf{Previous work}}
\\
\midrule

\citet{tang2013dner_tagging}
&&&
&80.0& 70.6& 75.0
&&&
\\

\citet{tang2018recognizing}
& 67.8 &64.9& 66.3
&&&
&&&
\\

\citet{metke2016concept}
& 64.4 & 56.5 & 60.2
&&&
&&&
\\
\citet{metke2016concept}*
&68.7& 66.1& 67.4
&77.0& 72.9& 74.9 
&74.9& 78.5& 76.6
\\

\citet{muis2016graph}*
& 72.1 & 48.4 & 58.0
& 83.9 & 60.4 & 70.3
& 79.1 & 70.7 & 74.7
\\

\citet{dai2020dner_transition}
& 68.9 & 69.0 & 69.0 
& 80.5 & 75.0 & 77.7
& 78.1 & 81.2 & 79.6
\\

\citet{wang2021dner_clique}
& 70.5 & 72.5 & 71.5
& 84.3 & 78.2 & 81.2
& 78.2 84.7 & 81.3
\\

\midrule
\multicolumn{10}{l}{\textbf{This work}} \\
\midrule
Forced alignment
& 69.1 & 71.6 & 70.3
& 82.9 & 80.6 & 81.7
& 79.4 & 85.4 & 82.3
\\
Soft EM & 70.9 & 72.2 & 71.5
 & 84.2 & 79.2 & 81.7
& 80.4 & 84.4 & 82.3
\\
Hard EM
& 69.6 & 71.2 & 70.4
& 83.6 & 79.6 & 81.5
& 77.7 & 85.3 & 81.3
\\
Soft EM + silver
& 69.4 & 69.8 & 69.6
& 82.7 & 80.7 & 81.7
& 79.1 & 84.7 & 81.8
\\
Hard EM + silver
& 72.1 & 72.5 & 72.3
& 84.2 & 79.6 & 81.8
& 80.5 & 84.4 & 82.4
\\
\bottomrule
\end{tabular}


==> tables/results_disc.tex <==

\begin{tabular}{@{}l@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{\hskip 0.3in}ccc@{}}
\toprule
& \multicolumn{3}{c}{\cadec} & \multicolumn{3}{c}{\sha} & \multicolumn{3}{c}{\shb} \\
\cmidrule(l{0pt}r{2pt}){2-4}\cmidrule(l{2pt}r{2pt}){5-7}\cmidrule(l{2pt}r{0pt}){8-10}
\\
& P & R & F1
& P & R & F1
& P & R & F1
\\

\midrule
\multicolumn{10}{l}{\textbf{Previous work}}
\\
\midrule



\citet{metke2016concept}
&&&
&&&
&&&
\\
\citet{metke2016concept}*
&5.8& 1.0& 1.8
&39.7& 12.3& 18.8 
&8.8& 4.5& 6.0
\\

\citet{muis2016graph}*
& 60.8 & 14.8 & 23.9
&  78.4& 36.6& 50.0
& 42.7&  39.5&  41.1
\\

\citet{dai2020dner_transition}
& 41.2 & 35.1 & 37.9
& 78.5 & 39.4 & 52.5
& 56.1 & 43.8 & 49.2
\\

\citet{wang2021dner_clique}
& 52.9 & 38.3 & 44.4
& 66.1 & 48.4 & 55.9
& 51.0 & 57.6 & 54.1
\\

\midrule
\multicolumn{10}{l}{\textbf{This work}} \\
\midrule
Forced alignment
& 36.6 & 39.4 & 38.0
& 52.0 & 50.7 & 51.3
& 54.5 & 61.1 & 57.6
\\
Soft EM
& 45.5 & 37.2 & 40.9
 & 55.4 & 49.1 & 52.1
& 55.8 & 55.8 & 55.8
\\
Hard EM
& 34.6 & 37.2 & 35.9
& 48.1 & 50.0 & 49.0
& 48.7 & 59.7 & 53.6
\\
Soft EM + silver
& 37.2 & 37.2 & 37.2
& 51.1 & 51.6 & 51.4
& 52.6 & 58.5 & 55.4
\\
Hard EM + silver & 45.5 & 42.5 & 44.0
& 56.1 & 48.6 & 52.1
& 51.5 & 56.5 & 53.9
\\
\bottomrule
\end{tabular}

